Low-rank Optimal Transport: Approximation, Statistics and Debiasing

The matching principles behind optimal transport (OT) play an increasingly important role in machine learning, a trend which can be observed when OT is used to disambiguate datasets in applications (e.g. single-cell genomics) or used to improve more complex methods (e.g. balanced attention in transformers or self-supervised learning). To scale to more challenging problems, there is a growing consensus that OT requires solvers that can operate on millions, not thousands, of points. The low-rank optimal transport (LOT) approach advocated in \cite{scetbon2021lowrank} holds several promises in that regard, and was shown to complement more established entropic regularization approaches, being able to insert itself in more complex pipelines, such as quadratic OT. LOT restricts the search for low-cost couplings to those that have a low-nonnegative rank, yielding linear time algorithms in cases of interest. However, these promises can only be fulfilled if the LOT approach is seen as a legitimate contender to entropic regularization when compared on properties of interest, where the scorecard typically includes theoretical properties (statistical complexity and relation to other methods) or practical aspects (debiasing, hyperparameter tuning, initialization). We target each of these areas in this paper in order to cement the impact of low-rank approaches in computational OT.

==> sections/contrib_diff.tex <==
\section{On the differentiability of Low-rank Optimal Transport}
In this section we aim at clarifying the differentation of $\text{LOT}_{r,c}$. Here we restrict ourselves to the discrete settings as it is the case of interest for practical use. Given $a$ and $b$ be respectively elements of $\Delta_n^*$ and $\Delta_m^*$ and  $\mathbf{X}\eqdef \{x_1,\dots,x_n\}$ and $\mathbf{Y} \eqdef \{y_1,\dots,y_m\}$ be respectively two subsets of $\mathcal{X}$ and $\mathcal{Y}$, recall that 
\begin{align*}
\text{LOT}_{r,c}(\mu_{a,\mathbf{X}},\nu_{b,\mathbf{Y}}) =   \min_{P\in\Pi_{a,b}(r)}\langle C,P\rangle\; .
\end{align*}
As $P\in\Pi_{a,b}(r)$ is a compact subset of $\mathbb{R}^{n\times m}$, and for any $P\in\Pi_{a,b}(r)$,  $C\in \mathbb{R}_{+}^{n\times m}\rightarrow \langle C,P\rangle$ is linear, one can apply Danskin's Theorem and obtain the subdifferiental of $C\in\mathbb{R}_{+}^{n\times m}\rightarrow \min_{P\in\Pi_{a,b}(r)}\langle C,P\rangle$ defined as
$$\partial\text{LOT}_{r,c}(C)=\left\{P\in\argmin_{P\in\Pi_{a,b}(r)}\langle C,P\rangle \right\}\; .$$

% If one wants to differentiate LOT w.r.t the masses, one needs to apply an implicit differentiation at each iteration of the outer loop.

% To differentiate the argmin: explain that we unroll the outerloop and apply an implicit differentiation of the dual of the MD update. In fact, because of $\alpha$, the dual admits a constraint therefore we consider another function, which at optimality coincide with the dual and apply the TFI on this function.



